BrickPal: Augmented Reality-based Assembly Instructions for Brick Models

The assembly instruction is a mandatory component of Lego-like brick sets.The conventional production of assembly instructions requires a considerable amount of manual fine-tuning, which is intractable for casual users and customized brick sets.Moreover, the traditional paper-based instructions lack expressiveness and interactivity.To tackle the two problems above, we present BrickPal, an augmented reality-based system, which visualizes assembly instructions in an augmented reality head-mounted display. It utilizes Natural Language Processing (NLP) techniques to generate plausible assembly sequences, and provide real-time guidance in the AR headset.Our user study demonstrates BrickPal's effectiveness at assisting users in brick assembly compared to traditional assembly methods. Additionally, the NLP algorithm-generated assembly sequences achieve the same usability with manually adapted sequences.

==> discussion.tex <==
\section{Discussion}

The technical evaluation and the user study reveal that the 3D-PALM is a simple but effective algorithm. However, it cannot generate the position and the brick at the same time. The position is not encoded intrinsically with the brick embedding but a separate token. It can be improved for the next version of 3D-PALM.

\begin{itemize}
    % \item Overall performance of the learning system
    \item Research questions in the user study
    \item The application scenario and Limitation of the hardware
    \item AI generated vs human generated
\end{itemize}

